LLM-based Vulnerability Discovery through the Lens of Code Metrics

Large language models (LLMs) excel in many tasks of software engineering, yet progress in leveraging them for vulnerability discovery has stalled in recent years. To understand this phenomenon, we investigate LLMs through the lens of classic code metrics. Surprisingly, we find that a classifier trained solely on these metrics performs on par with state-of-the-art LLMs for vulnerability discovery. A root-cause analysis reveals a strong correlation and a causal effect between LLMs and code metrics: When the value of a metric is changed, LLM predictions tend to shift by a corresponding magnitude. This dependency suggests that LLMs operate at a similarly shallow level as code metrics, limiting their ability to grasp complex patterns and fully realize their potential in vulnerability discovery. Based on these findings, we derive recommendations on how research should more effectively address this challenge.

==> tikz/correlation.tex <==
\scalebox{0.70}{
\begin{tikzpicture}[scale=0.42]
  \foreach \y [count=\n] in {
       { 1.000, 0.145, 0.089, 0.112, 0.127, 0.074, 0.104, 0.162, 0.090, 0.187, 0.003, 0.006, 0.024, 0.016, 0.034, 0.038, 0.015, 0.008, 0.000, 0.026, 0.000, 0.004, 0.006 },
{ 0.145, 1.000, 0.098, 0.109, 0.163, 0.044, 0.103, 0.071, 0.102, 0.036, 0.022, 0.053, 0.092, 0.101, 0.081, 0.094, 0.022, 0.034, 0.000, 0.012, 0.000, 0.000, 0.011 },
{ 0.089, 0.098, 1.000, 0.708, 0.317, 0.213, 0.230, 0.132, 0.212, 0.058, 0.044, 0.075, 0.233, 0.159, 0.200, 0.202, 0.058, 0.049, 0.006, 0.037, 0.000, 0.016, 0.005 },
{ 0.112, 0.109, 0.708, 1.000, 0.388, 0.298, 0.266, 0.184, 0.265, 0.081, 0.040, 0.071, 0.213, 0.146, 0.194, 0.181, 0.061, 0.040, 0.005, 0.046, 0.000, 0.013, 0.006 },
{ 0.127, 0.163, 0.317, 0.388, 1.000, 0.313, 0.256, 0.243, 0.284, 0.099, 0.039, 0.063, 0.176, 0.153, 0.178, 0.168, 0.075, 0.029, 0.002, 0.035, 0.000, 0.007, 0.008 },
{ 0.074, 0.044, 0.213, 0.298, 0.313, 1.000, 0.160, 0.214, 0.276, 0.087, 0.039, 0.064, 0.158, 0.107, 0.057, 0.105, 0.009, 0.016, 0.004, 0.038, 0.000, 0.012, 0.003 },
{ 0.104, 0.103, 0.230, 0.266, 0.256, 0.160, 1.000, 0.158, 0.233, 0.081, 0.026, 0.049, 0.166, 0.107, 0.188, 0.103, 0.059, 0.035, 0.002, 0.037, 0.001, 0.024, 0.023 },
{ 0.162, 0.071, 0.132, 0.184, 0.243, 0.214, 0.158, 1.000, 0.364, 0.355, 0.006, 0.019, 0.061, 0.043, 0.052, 0.072, 0.013, 0.009, 0.000, 0.022, 0.000, 0.004, 0.005 },
{ 0.090, 0.102, 0.212, 0.265, 0.284, 0.276, 0.233, 0.364, 1.000, 0.135, 0.021, 0.061, 0.169, 0.118, 0.129, 0.151, 0.022, 0.029, 0.000, 0.037, 0.000, 0.010, 0.009 },
{ 0.187, 0.036, 0.058, 0.081, 0.099, 0.087, 0.081, 0.355, 0.135, 1.000, 0.002, 0.005, 0.020, 0.013, 0.019, 0.028, 0.005, 0.004, 0.000, 0.011, 0.001, 0.002, 0.003 },
{ 0.003, 0.022, 0.044, 0.040, 0.039, 0.039, 0.026, 0.006, 0.021, 0.002, 1.000, 0.556, 0.206, 0.325, 0.090, 0.042, 0.014, 0.036, 0.212, 0.011, 0.000, 0.000, 0.000 },
{ 0.006, 0.053, 0.075, 0.071, 0.063, 0.064, 0.049, 0.019, 0.061, 0.005, 0.556, 1.000, 0.323, 0.483, 0.140, 0.094, 0.024, 0.038, 0.120, 0.020, 0.000, 0.009, 0.000 },
{ 0.024, 0.092, 0.233, 0.213, 0.176, 0.158, 0.166, 0.061, 0.169, 0.020, 0.206, 0.323, 1.000, 0.565, 0.270, 0.242, 0.049, 0.053, 0.030, 0.023, 0.061, 0.054, 0.007 },
{ 0.016, 0.101, 0.159, 0.146, 0.153, 0.107, 0.107, 0.043, 0.118, 0.013, 0.325, 0.483, 0.565, 1.000, 0.213, 0.172, 0.048, 0.059, 0.051, 0.025, 0.000, 0.000, 0.000 },
{ 0.034, 0.081, 0.200, 0.194, 0.178, 0.057, 0.188, 0.052, 0.129, 0.019, 0.090, 0.140, 0.270, 0.213, 1.000, 0.148, 0.078, 0.060, 0.013, 0.017, 0.001, 0.027, 0.011 },
{ 0.038, 0.094, 0.202, 0.181, 0.168, 0.105, 0.103, 0.072, 0.151, 0.028, 0.042, 0.094, 0.242, 0.172, 0.148, 1.000, 0.042, 0.025, 0.012, 0.038, 0.125, 0.033, 0.009 },
{ 0.015, 0.022, 0.058, 0.061, 0.075, 0.009, 0.059, 0.013, 0.022, 0.005, 0.014, 0.024, 0.049, 0.048, 0.078, 0.042, 1.000, 0.020, 0.008, 0.008, 0.000, 0.002, 0.001 },
{ 0.008, 0.034, 0.049, 0.040, 0.029, 0.016, 0.035, 0.009, 0.029, 0.004, 0.036, 0.038, 0.053, 0.059, 0.060, 0.025, 0.020, 1.000, 0.000, 0.011, 0.000, 0.002, 0.002 },
{ 0.000, 0.000, 0.006, 0.005, 0.002, 0.004, 0.002, 0.000, 0.000, 0.000, 0.212, 0.120, 0.030, 0.051, 0.013, 0.012, 0.008, 0.000, 1.000, 0.000, 0.000, 0.000, 0.000 },
{ 0.026, 0.012, 0.037, 0.046, 0.035, 0.038, 0.037, 0.022, 0.037, 0.011, 0.011, 0.020, 0.023, 0.025, 0.017, 0.038, 0.008, 0.011, 0.000, 1.000, 0.000, 0.020, 0.006 },
{ 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 0.001, 0.000, 0.000, 0.001, 0.000, 0.000, 0.061, 0.000, 0.001, 0.125, 0.000, 0.000, 0.000, 0.000, 1.000, 0.000, 0.000 },
{ 0.004, 0.000, 0.016, 0.013, 0.007, 0.012, 0.024, 0.004, 0.010, 0.002, 0.000, 0.009, 0.054, 0.000, 0.027, 0.033, 0.002, 0.002, 0.000, 0.020, 0.000, 1.000, 0.044 },
{ 0.006, 0.011, 0.005, 0.006, 0.008, 0.003, 0.023, 0.005, 0.009, 0.003, 0.000, 0.000, 0.007, 0.000, 0.011, 0.009, 0.001, 0.002, 0.000, 0.006, 0.000, 0.044, 1.000 },
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \pgfmathsetmacro{\twox}{\x*160}
        \node[fill=poscolor!\twox!white, minimum size=4.4mm, text=white] at (\m,-\n) { };
      }
    }

  % column labels
  \foreach \a [count=\i] in {T2,C7,M2,M3,C8,C10,C11,C3,C2,C4,S5,C1,T1,C6,S4,S1,C9,M1,S2,C12,T3,S3,C5} {
    \node[minimum size=6mm, rotate=90, anchor=west] at (\i, 0) {\a};
  }
  % row labels
  \foreach \a [count=\i] in {T2,C7,M2,M3,C8,C10,C11,C3,C2,C4,S5,C1,T1,C6,S4,S1,C9,M1,S2,C12,T3,S3,C5} {
    \node[minimum size=6mm, xshift=0.0cm, anchor=east] at (0,-\i) {\a};
  }
  
  % Cluster 1
  \draw[black!80, dashed] (7.5, -7.5) rectangle (10.5, -10.5);
  % Cluster 2
  \draw[black!80, dashed] (10.5, -10.5) rectangle (14.5, -14.5);
  % Cluster 3
  \draw[black!80, dashed] (2.5, -2.5) rectangle (4.5, -4.5);

  % Main cluster
  \draw[black!80, dashed] (0.5, -0.5) rectangle (16.5, -16.5);
  
  % Adding the legend
  % \draw[top color=poscolor!160!white, minimum size=6mm, color=white] (24, -9.5) rectangle (25.00, -14.5);
  \draw[top color=poscolor!160!white, minimum size=6mm, color=white] (24.5, -7.5) rectangle (25.5, -15.5);

  % Adding text nodes to the top and bottom of the red rectangle
  % \node[anchor=south] at (24.5, -9.5) {1.0};
  % \node[anchor=north] at (24.5, -14.5) {0.0};
  \node[anchor=south] at (25, -7.5) {1.0};
  \node[anchor=north] at (25, -15.5) {0.0};
\end{tikzpicture}}

\vspace{-2pt}

\hspace{-14pt}
\scalebox{0.70}{
\begin{tikzpicture}[scale=0.42]
  \foreach \y [count=\n] in {
       {0.0351, 0.0096, 0.0259, 0.0320, 0.0335, 0.0302, 0.0291, 0.0299, 0.0281, 0.0279, 0.0047, 0.0056, 0.0125, 0.0092, 0.0189, 0.0113, 0.0100, 0.0063, 0.0047, 0.0030, 0.0004, 0.0008, 0.0055},
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \pgfmathsetmacro{\twox}{\x*1200}
        \node[fill=negcolor!\twox!white, minimum size=4.4mm, text=white] at (\m,-\n) { };
      }
    }

  % row labels
  \foreach \a [count=\i] in {y} {
    \node[minimum size=6mm, xshift=0.0cm, anchor=east] at (0,-\i) {\a};
  }
  
  % Adding the legend
  \draw[left color=white, right color=negcolor!120!white, minimum size=6mm, color=white] (8.0, -2.5) rectangle (16.0, -3.5);

  % Adding text nodes to the top and bottom of the red rectangle
  \node[anchor=north] at (7.0, -2.4) {0.};
  \node[anchor=north] at (17.0, -2.4) {0.1};
\end{tikzpicture}}

==> tikz/metric_analysis.tex <==
\begin{tikzpicture}
\begin{axis}[
xlabel={\# Metrics},
ylabel={\% of F1},
axis x line*=bottom,
axis y line*=left,
xtick={1,5,10,15,20},
ymin=80,
%ymax=100,
xmin=1,
xmax=23,
width=\linewidth,
height=0.60\linewidth,
grid=major,
legend cell align={left},
legend style={at=({0.993,0.075}),anchor=south east},
%legend style={draw=none, fill=none},
%legend entries={
%    {\textcolor{poscolor}{SCM}},
%    {\textcolor{negcolor}{UniXcoder}},
%},
%legend pos=south east,
]
\addplot [name path=lower, fill=none, draw=none, forget plot] table [
    x index=0,
    y expr=\thisrowno{1} - \thisrowno{2}]{data/metric_analysis/best_metrics.dat};
\addplot [name path=upper, fill=none, draw=none, forget plot] table [
    x index=0,
    y expr=\thisrowno{1} + \thisrowno{2}]{data/metric_analysis/best_metrics.dat};
\addplot[poscolor!70, opacity=0.5, forget plot] fill between[of=lower and upper];
\addplot [poscolor] table {data/metric_analysis/best_metrics.dat};
\addlegendentry{\small{\ SCM}}

%\addplot [name path=trainlower, fill=none, draw=none, forget plot] table [
%    x index=0,
%    y expr=\thisrowno{1} - \thisrowno{2}]{data/metric_analysis/best_metrics_train.dat};
%\addplot [name path=trainupper, fill=none, draw=none, forget plot] table [
%    x index=0,
%    y expr=\thisrowno{1} + \thisrowno{2}]{data/metric_analysis/best_metrics_train.dat};
%\addplot[poscolor!70, opacity=0.5, forget plot] fill between[of=trainlower and trainupper];
%\addplot [poscolor] table {data/metric_analysis/best_metrics_train.dat};
%\addlegendentry{\small{SCM}}

%\addplot [name path=sotalower, fill=none, draw=none, forget plot] coordinates {(0, 20.43) (23, 20.43)};
%\addplot [name path=sotaupper, fill=none, draw=none, forget plot] coordinates {(0, 21.236) (23, 21.23)};
%\addplot[negcolor!70, opacity=0.5, forget plot] fill between[of=sotalower and sotaupper];
%\addplot [negcolor] coordinates {(0, 20.83) (23, 20.83)};
%\addlegendentry{\small{UniXcoder}}
\end{axis}
\end{tikzpicture}
